Transformer-Transducers for Code-Switched Speech Recognition

We live in a world where 60% of the population can speak two or more languages fluently. Members of these communities constantly switch between languages when having a conversation. As automatic speech recognition (ASR) systems are being deployed to the real-world, there is a need for practical systems that can handle multiple languages both within an utterance or across utterances. In this paper, we present an end-to-end ASR system using a transformer-transducer model architecture for code-switched speech recognition. We propose three modifications over the vanilla model in order to handle various aspects of code-switching. First, we introduce two auxiliary loss functions to handle the low-resource scenario of code-switching. Second, we propose a novel mask-based training strategy with language ID information to improve the label encoder training towards intra-sentential code-switching. Finally, we propose a multi-label/multi-audio encoder structure to leverage the vast monolingual speech corpora towards code-switching. We demonstrate the efficacy of our proposed approaches on the SEAME dataset, a public Mandarin-English code-switching corpus, achieving a mixed error rate of 18.5% and 26.3% on test_man and test_sge sets respectively.

==> tables/dataset_split.tex <==
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
 & train & dev & test$_{man}$ & test$_{sge}$ \\
\midrule
\multicolumn{5}{c}{\textsc{SEAME code-switched data}}\\
\midrule
Speakers & 128 & 6 & 10 & 10 \\
Duration (hrs) & 93.0 & 4.7 & 7.5 & 3.9 \\
\midrule
\multicolumn{5}{c}{\textsc{TEDLIUMv2 English monolingual data}}\\
\midrule
Duration & \multicolumn{4}{c}{211 hours (1267 speakers)} \\
\midrule
\multicolumn{5}{c}{\textsc{AISHELL-1 Mandarin monolingual data}}\\
\midrule
Duration & \multicolumn{4}{c}{150 hours (340 speakers)} \\
 \bottomrule
\end{tabular}
% }
